Ultrasound Lung Aeration Map via Physics-Aware Neural Operators

Lung ultrasound is a growing modality in clinics for diagnosing and monitoring acute and chronic lung diseases due to its low cost and accessibility. Lung ultrasound works by emitting diagnostic pulses, receiving pressure waves and converting them into radio frequency (RF) data, which are then processed into B-mode images with beamformers for radiologists to interpret. However, unlike conventional ultrasound for soft tissue anatomical imaging, lung ultrasound interpretation is complicated by complex reverberations from the pleural interface caused by the inability of ultrasound to penetrate air. The indirect B-mode images make interpretation highly dependent on reader expertise, requiring years of training, which limits its widespread use despite its potential for high accuracy in skilled hands. To address these challenges and democratize ultrasound lung imaging as a reliable diagnostic tool, we propose LUNA, an AI model that directly reconstructs lung aeration maps from RF data, bypassing the need for traditional beamformers and indirect interpretation of B-mode images. LUNA uses a Fourier neural operator, which processes RF data efficiently in Fourier space, enabling accurate reconstruction of lung aeration maps. LUNA offers a quantitative, reader-independent alternative to traditional semi-quantitative lung ultrasound scoring methods. The development of LUNA involves synthetic and real data: We simulate synthetic data with an experimentally validated approach and scan ex vivo swine lungs as real data. Trained on abundant simulated data and fine-tuned with a small amount of real-world data, LUNA achieves robust performance, demonstrated by an aeration estimation error of 9% in ex-vivo lung scans. We demonstrate the potential of reconstructing lung aeration maps from RF data, providing a foundation for improving lung ultrasound reproducibility and diagnostic utility.

==> sections/Xintro_old.tex <==
\begin{figure}[t!]
    \centering
   \includegraphics[width=0.79\columnwidth]{figures/fig1_teaser.pdf}
    \caption{{\bf Overview: LungNO (the lung ultrasound neural operator) can reconstruct lung aeration maps from ultrasound radio-frequency (RF) data}. %\todo{GIVE it a name as a graph abstract.}%  from commercially-available ultrasound probes and research machine. 
 {\bf a}, Our machine learning (ML) model, LungNO, can reconstruct lung aeration maps from lung ultrasound (LUS) RF data.
 Ultrasound devices scan the lung and 
 %A subject's lung is scanned with an ultrasound probe and 
 the RF data is fed to ML for reconstructing a lung air-tissue map, or aeration map, which is human-interpretable. The aeration map is used to estimate lung percent aeration, a critical clinical outcome for evaluation, monitoring and diagnostics. %that enables clinical diagnosis, monitoring and intervention.
%We study the inverse problem of lung ultrasound (LUS) imaging, i.e. reconstructing lung histology maps from ultrasound radio frequency (RF) data. RF data and lung histology pairs are derived with full-wave propagation physics with Fullwave-2 \cite{pinton2021fullwave} which simulates the scanning of porcine lung specimens with an ultrasound device. We develop a machine learning model to reconstruct the lung histology from RF data. 
{\bf b}, The forward process of ultrasound wave propagation in the lung, whose physics simulation generates the training data for LungNO.
{\bf c}, The inverse problem of reconstructing the lung aeration map $\rho^A$ from RF data $p$ is challenging due to the ill-posedness. We propose a deep neural operator framework, LungNO, as a surrogate model to solve the inverse problem.
{\bf d/e}, Existing v.s. our method. The current practice, B-mode lung image screening, visualizes RF data via beamforming ({\bf d}). Due to the complexity of the wave propagation physics in the lung, which exhibits complicated tissue-air structures and varying imaging parameters like dynamic range, b-mode images are hard to interpret and need years of experience. In contrast, we reconstruct lung aeration maps that directly depict tissue-air structures, which are interpretable for important clinical signs like percent aeration ({\bf e}).
{\bf f}, We validate LungNO's performance on ex vivo data. Swine lung tissues are scanned and the LUS RF data is fed to LungNO for estimating lung percent aeration, which is compared and validated with the ground truth.
%\pw{@Todo: add a visualization of full wave to generate new images.}
    }
    \label{fig:teaser}
\end{figure}


\section{Introduction}


%\pw{to refine intro: Enable diagnostics beyond what is possible from radiologists, because we learn to model the fundamental physicist in lung. We recover what is not available or not sensitive to radiologists.

%\pw{Lung ultrasound imaging: Background and impacts. Current limitations.}
Lung ultrasound (LUS) is an important non-invasive real-time imaging method widely used for diagnostic assessment of lung conditions in patients with respiratory and extrapulmonary diseases \cite{bouhemad2015ultrasound,lacedonia2021role,manolescu2020ultrasound}. Unlike other modalities, e.g. X-ray imaging and computed tomography (CT), LUS has the inherent advantages of being non-ionizing, low-cost, portable and can be indicated for frequent or continuous bedside monitoring. Furthermore, the acoustic soft-tissue/air interaction provides a fundamentally different source of contrast, potentially providing information that is complementary to X-ray imaging methods \cite{lichtenstein2014lung}.
Modern clinical LUS employs brightness-mode images (B-mode images) based on visualization of diagnostic pulse reflections from tissue inhomogeneities, including tissue-air interfaces. Beamforming is a process to transform a set of received radio frequency (RF) signals (function of time) into human-readable B-mode images representing anatomical lung structures in space, where the pixel brightness is dependent on the magnitude of received reflection.
%For the convenience of clinical screening, high-dimensional lung ultrasound data is compressed to two dimensions and beamforms a brightness-mode image, or B-mode image, in which tissues of interest are depicted as points of variable brightness.
%The interpretation of LUS B-mode images plays a key role in the diagnosis \cite{lichtenstein2014lung,gargani2014lung}.
However, unlike other diagnostic ultrasound (e.g. fetal and abdominal ultrasound \cite{whitworth2015ultrasound,mattoon2014abdominal}), the brightness of an LUS B-mode image does not directly represent tissue echogenicity, as ultrasound cannot penetrate through the tissue-air interface \cite{soldati2020}.
Reproducibility and interpretability of clinical LUS are limited and depend not only on the radiologist/reader's experience but also on the equipment (probe and machine) and its parameters (central frequency, focal depth, TGC, spatial compounding, harmonic imaging), which is manifested in insufficient interobserver agreement \cite{pivetta2018sources,gomond2020effect,gravel2020interrater,kumar2021,fatima2023}, posing significant changes for LUS-based diagnosis.

%\todo{Background of why aeration map is more important:Among different lung diseases, we focus on the case of air replaced by fluid, which typically occurs in the acute phases of disease, e.g., in ARDS.  This case is most sensitive to lung ultrasound and can be reflected by the lung aeration map. The main goal of the paper is to reconstruct aeration maps from lung ultrasound RF data.
%We consider the case when air is replaced by fluid in lung, which typically occurs in the acute phases of disease, e.g., in ARDS. It has significant acoustical effect and more detectable by LUS.
% Lung histopathology images were binary segmented (air/non-air components) to form aeration maps.}
Recently, machine learning models have been developed for LUS and are considered to be a helpful tool that assists clinicians for LUS image interpretation and diagnostic purposes \cite{xing2023,sagreiya2023}. %can help reduce the need for human interpretation in LUS. 
Such methods take B-mode images as input and learn to identify the image features like horizontal (A-lines) and vertical (B-lines) artifacts \cite{zhao2024detection,hou2020interpretable}, or directly classify the disease, including COVID-19 and pneumonia \cite{horry2020covid,born2020pocovid,roy2020deep}.
Though successful, a machine learning model that directly reads and learns from B-mode images face several challenges: 1) the information related to lung morphology at mesoscopic/alveolar level is lost in the beamforming process \cite{mento2024}; 2) such models do not generalize well to different ultrasound devices as each device has a setting with different imaging parameters %due to the wide use of a variety of parameter  settings 
(dynamic range, time gain compensation) and quality of the resulting B-mode images also vary \cite{xu2023}.%could have domain gaps.
%1) machine variability; 2) 
%has emerged as an important real-time imaging method that combines the evaluation of lung morphology and function, including in critically ill patients.
%LUS b-mode images are commonly used in clinics. However, they are hard to interpret \cite{} and hinder accurate disease diagnosis. 
%On the other hand, lung histology can accurately reflect lung aeration status but hard to reconstruct in LUS.



Our work is a departure from mainstream approaches towards LUS analysis: rather than interpreting B-mode images, either manually or automatically \cite{lichtenstein2014lung,lee2014lung,baloescu2020automated}, our model directly reconstructs lung aeration maps from raw RF data, which recovers features in LUS that are not available or not sensitive to radiologists.
Specifically, we propose a model that reconstructs lung aeration maps from delayed RF data, bypassing the traditional reliance on B-mode images and has two major advantages: 
{1)} We directly take raw ultrasound RF data as the input and avoid the information loss in the beamforming process and the variability caused by different device/beamforming settings. 
{2)} We directly reconstruct lung aeration maps, which avoids the necessity of interpreting B-mode images.
The reconstructed lung aeration map enables the calculation of the lung percent aeration, a critical clinical measurement for diagnosis \cite{lee2020lung,kalkanis2022lung}. We validate the estimated percent aeration both {\it in silico} and {\it ex vivo}, demonstrating the efficacy of our approach.




We address  two major challenges in developing a machine learning model to solve the inverse problem and reconstruct lung aeration maps reconstruction from RF data: 
{ 1)} the problem is highly ill-posed due to the complicated ultrasound propagation physics in the lung with complex highly reflective structures, and efficient learning and detecting tiny changes in RF data is pivotal;
{ 2)} Obtaining abundant real pairs of lung RF data and corresponding aeration map is challenging because lung imaging (e.g. CT) is difficult due to factors such as fast-changing lung shape with inspiration. Additionally, matching lung images of other modalities with LUS is hard. % and complex tissue-air structures.
Our method highlights technical novelties that aim to alleviate these issues:
{ 1)} Our machine learning framework for LUS is based on Fourier neural operator (FNO) \cite{li2021fourier}, which has empirically achieved good performance across various applications, such as material science~\cite{rashid2022learning}, weather forecasting~\cite{pathak2022fourcastnet} and photoacoustic imaging~\cite{guan2023fourier}. FNO allows parameterizing directly in Fourier space and is more efficient for processing RF data. We refer to the framework as LungNO (the lung ultrasound neural operator) in the paper.
{ 2)} For the scarcity of the real data, we train on the abundant simulated data %(based on Fullwave-2 \cite{pinton2021fullwave} which simulates full-wave propagation physics) 
and fine-tune on a small number of real data samples. The model reconstructs lung aeration maps from simulation and performs well in real data.
%There are challenges and there exist no prior works: 1) ill-pose; 2) complicated physics.

%It is of interest to reconstruct lung histology from the LUS radiofrequency data and enable clinical feature estimation such as aeration.

%[What is the problem?]
%Lung histopathology from ultrasound data.

%What others have done?
%B-mode images. No optimization pipeline.

%What is the gap?
%\begin{enumerate}
%    \item bmode: Low res, hard to interpret/diagnose, rely on operator's skills/experience
%    \item inverse problem: not possible to the ill-pose nature and time/cost needed
%\end{enumerate}

%What we've done?
%ML to learn the inverse mapping


%Contribution
%1) impact;
%2) technical novelties 
%- physics-aware network design
%- uncertainty
%- other small details: MS co-training, masking loss (as data augmentation)

%Background and the impact of lung ultrasound imaging from RF data.

To summarize, the proposed LungNO has two main contributions:
\begin{itemize}
\item {\bf Pioneering ultrasound lung aeration map reconstruction.} This work is the first to reconstruct lung aeration maps from ultrasound RF data, enabling accurate percent aeration estimation and supporting future diagnostic applications.
 \item  {\bf Effectiveness of simulation data and its generalizability to real scenarios.} 
We demonstrate the power of learning wave propagation physics in lung using simulation: Training on abundant simulation data, our model demonstrates satisfactory generalizability on \textit{ex vivo} data. %. Our direct evaluation on real data highlights the satisfactory generalizability of our approach.
\item \reader{{\bf Improvement for radiologist reading}. Our method has been shown to improve the reader's accuracy and efficiency for radiologists in clinical settings (pending on reader study)}
%\item \textbf{Masking Loss as Data Augmentation}. Simulations are time and resource consuming. We randomly mask input regions as data augmentation and increase the robustness of the learning algorithm. 
%\item {\bf Uncertainty measurement} that allows the confidence of the prediction.

\end{itemize}

\begin{figure}[t!]
    \centering
   \includegraphics[width=0.95\columnwidth]{figures/fig1.pdf}% $fig1_teaser.pdf}
    \caption{\small {\bf Overview: \method (the Lung Ultrasound Neural operator for Aeration map) reconstructs lung aeration maps from ultrasound radio-frequency (RF) data}. 
 {\bf a}, %\method reconstructs lung aeration maps from lung ultrasound (LUS) RF data.
 The imaging process: Ultrasound devices scan the lung and 
 %A subject's lung is scanned with an ultrasound probe and 
 the RF data is fed to \method for reconstructing a lung air-tissue map, or aeration map, which is human-interpretable. The aeration map is used to estimate lung percent aeration, a critical clinical outcome for evaluation, monitoring and diagnostics \cite{lee2020lung,kalkanis2022lung}. 
%{\bf c}, The inverse problem of reconstructing the lung aeration map $\rho^A$ from RF data $p$ is challenging due to the ill-posedness. We propose a deep neural operator framework, \method, as a surrogate model to solve the inverse problem.
{\bf Existing v.s. our approach:} The current practice, B-mode lung image (upper right) requires manual interpretation of artifacts like B lines to assign LUS score \cite{volpicelli2012international}, which has high variations due to the difficulty of identifying artifacts created by the complex wave propagation physics in the lung. LUS score is also coarse, image-level and semi-quantitative.
%screening, visualizes RF data via beamforming. 
%Due to the complexity of the wave propagation physics in the lung, which exhibits complicated tissue-air structures and varying imaging parameters like dynamic range, b-mode images are hard to interpret and have high variations. 
{\bf Our approach} (lower right): We reconstruct lung aeration maps that directly depict tissue-air maps, from which clinicians can directly read pixel-level aeration. The method is reproducible and provides quantitative two-dimensional aeration distribution.
%which are interpretable for important clinical signs like percent aeration 
%{\bf f}, We validate \method's performance on ex vivo data. Swine lung tissues are scanned and the LUS RF data is fed to \method for estimating lung percent aeration, which is compared and validated with the ground truth.
{\bf b,} \method performance on synthetic lung ultrasound data. Pixel-level aeration can be read from the predicted aeration map, which is visually similar to the true aeration map.
{\bf c,} \method performance on real ex-vivo lung ultrasound data. The average aeration prediction error is 9.4\%.
  %{\bf b/c,} \method percent aeration prediction performance of \textit{ex vivo} data. The prediction and ground truth are close to the perfect prediction line, suggesting its capability to estimate lung aeration ex vivo.
    }
    \label{fig:teaser}
\end{figure}
